Unseen Horizons: Unveiling the Real Capability of LLM Code Generation Beyond the Familiar

Recently, large language models (LLMs) have shown strong potential in code generation tasks. However, there are still gaps before they can be fully applied in actual software development processes. Accurately assessing the code generation capabilities of large language models has become an important basis for evaluating and improving the models. Some existing works have constructed datasets to evaluate the capabilities of these models. However, the current evaluation process may encounter the illusion of "Specialist in Familiarity", primarily due to three gaps: the exposure of target code, case timeliness, and dependency availability. The fundamental reason for these gaps is that the code in current datasets may have been extensively exposed and exercised during the training phase, and due to the continuous training and development of LLM, their timeliness has been severely compromised. The key to solve the problem is to, as much as possible, evaluate the LLMs using code that they have not encountered before. Thus, the fundamental idea in this paper is to draw on the concept of code obfuscation, changing code at different levels while ensuring the functionality and output. To this end, we build a code-obfuscation based benchmark OBFUSEVAL. We first collect 1,354 raw cases from five real-world projects, including function description and code. Then we use three-level strategy (symbol, structure and semantic) to obfuscate descriptions, code and context dependencies. We evaluate four LLMs on OBFU- SEVAL and compared the effectiveness of different obfuscation strategy. We use official test suites of these projects to evaluate the generated code. The results show that after obfuscation, the average decrease ratio of test pass rate can up to 62.5%.

==> backgroundCopy.tex <==
\section{BACKGROUND}
\label{sec:related}

%devEval 李戈那篇论文里有个可以打的点，就是他们在给上下文的时候，是目标代码里用了哪些依赖就直接给了哪些依赖，这是很强的提示了，没有像我们那样给一部分无用的依赖来作为混淆。
%CoderEval 和humaneval的比较没有考虑代码长度的影响，代码长度本身就会对模型的能力产生影响，不能说明他的benchmark更好。
%所以我们的实验结果中可以按照代码行的长度来进行划分，按照依赖的数量来进行划分。
%而且CodeEval和devEval都是只重写了功能描述，描述匹配代码是容易的，不能说明benchmark好


%%%%在这里介绍强调与那些算法题数据集的区别


In this section, we first conduct a comprehensive examination of the latest advancements in Large Language Models (LLMs) within code generation.   Subsequently, we delve into the evaluations crafted for code generation, along with the limitations and challenges encountered in assessing the performance of LLMs.   Finally, we underscore the novelty of our research in this evolving field. 
%在这一部分中，我们首先全面审视了大型语言模型（LLMs）在代码生成方面的最新进展，然后我们还分析了针对代码生成的测评工作，以及它们在评估LLMs性能时所遇到的局限性和挑战。最后，我们强调了我们研究的新颖性。

\subsection{Large Language Models for Code Generation.}

The process of code generation, which involves the automatic creation of complete program code or the completion of code snippets from higher-level representations, such as natural language descriptions, models, or specifications, plays a pivotal role in enhancing programming efficiency and mitigating human error~\cite{budinsky1996automatic,svyatkovskiy2020intellicode,parvez2021retrieval}. 
Recent advancements in Large Language Models (LLMs) for code generation have garnered significant attention in the realm of computer science research. These LLMs, such as GPT-4 ~\cite{GPT-4}, ChatGLM~\cite{du2021glm}, CODEX ~\cite{chen2021evaluating}, and CodeGen~\cite{nijkamp2022codegen}, have demonstrated remarkable capabilities not only in general natural language processing tasks ~\cite{chang2023survey} but also in the specific area of code generation. Notably, GPT-4 achieved the highest pass rate on the HumanEval benchmark~\cite{chen2021evaluating}, indicating a growing trend to evaluate the code generation capacity of general LLMs ~\cite{shen2023pangu}.

Code-specific LLMs, which are trained primarily on massive code-specific corpora, often outperform general LLMs in code generation tasks~\cite{zan2023large,luo2023wizardcoder,shen2023pangu}. Diverse training approaches have been employed, with some models like InCoder ~\cite{fried2022incoder} and StarCoder~\cite{li2023starcoder} being trained with the "filling-in-the-middle" capability for infilling missing code based on context. A variety of code LLMs have been proposed, such as WizardCoder~\cite{luo2023wizardcoder}, Instruct-StarCoder ~\cite{Instruct-starcoder}, and Instruct-CodeGen~\cite{Instruct-codegen}, each designed with different training objectives.      



\subsection{Evaluations for Code Generation}


When evaluating the code generation capabilities of LLMs, existing studies and benchmarks focus on the functional correctness of the code, which is usually verified by executing test cases. We propose ConfuEval, which is currently the only benchmark that performs rewrite obfuscation of code based on real project code, to assess the syntactic and functional correctness of LLMs-generated code by compilation pass rate and test pass rate, respectively. Further rewrite obfuscation based on real project code is crucial but also presents challenges. First, ensuring that the selected project can be successfully compiled and sandboxed is essential for a successful implementation, however, this is not easily achieved in many existing open-source projects. Second, builders need a deep understanding of the complex logic of the project to rewrite the code.

Traditional benchmarking focuses on generating independent code units, ignoring the contextual relationships between code~\cite{chen2021evaluating,austin2021program,zheng2023codegeex,li2022competition,yu2018spider}. However, current studies indicate that only about 30\% of methods in open-source projects are relatively independent~\cite{yu2024codereval} in real-world scenarios, methods often depend on each other or share variables, which is not considered in these traditional benchmarks. Therefore, we need evaluation methods that are closer to real-world scenarios to comprehensively assess the performance of LLMs in real software development.

Current benchmarks built based on real projects usually rewrite only the functional descriptions without modifying the code itself~\cite{yu2024codereval,li2024deveval}, which may lead to unfair evaluations as the model may memorize or copy the target code directly from the training data. Although SWE-BENCH~\cite{jimenez2023swe} collects modified code from the project's history, the code may still be something the model has seen before due to the presence of code clones. In addition, benchmarking that relies solely on the history also suffers from the problem of timeliness to evaluate subsequent releases of the model. In addition, SWE-BENCH does not provide the complete set of dependencies that a large language model needs to generate code, instead leaving the model to search for them on its own, so it is impossible to distinguish between a large language model's poorer ability to search for dependencies or its poorer ability to generate code itself. On the other hand, codereval~\cite{yu2024codereval} and DevEval~\cite{li2024deveval} provide complete dependencies but do not include useless and obfuscated dependencies, so the dependencies provided in this way may guide the big models in generating code, leading to unfair test results. In addition, previous benchmark tests were compared to Humaneval to prove their validity. However, since the length of code to be generated by these benchmark tests does not match the distribution of code lengths in Humaneval~\cite{du2023classeval,li2024deveval,yu2024codereval}, this comparison is inherently unfair and therefore does not accurately reflect the validity of the benchmark tests. 

\begin{comment}

在评估LLMs的代码生成能力时，已有的研究和基准主要集中在代码的功能正确性上，通常通过执行测试用例进行验证。我们提出的ConfuEval是目前唯一一个在真实项目代码基础上对代码进行重写混淆的基准测试，通过编译通过率和测试通过率分别评估大型模型生成代码的语法和功能正确性。在真实项目代码上的基础上进一步进行重写混淆至关重要，但也面临着挑战。首先，确保所选项目能够成功编译和沙箱化对于成功执行是必不可少的，然而，这在许多现有开源项目中并不容易实现。其次，构建者需要对项目的复杂逻辑有深入理解才能对代码进行改写。

传统基准测试主要关注生成独立的代码单元，而忽略了代码之间的上下文关系。然而，在实际场景中，方法通常相互依赖或共享变量，这种情况在这些传统基准测试中未被考虑。因此，我们需要更贴近实际场景的评估方法来全面评估大型语言模型在真实软件开发中的性能。

目前基于真实项目构建的基准测试通常只重写功能描述而未修改代码本身，这可能导致评估不公平，因为模型可能直接从训练数据中记忆或复制目标代码。虽然SWE-BENCH是从项目的历史记录中收集了修改后的代码，但由于存在代码克隆等原因，这些代码可能仍然是模型曾经见过的。此外，仅依赖于历史记录的基准测试也存在时效性问题，无法评估后续发布的模型。此外，SWE-BENCH未提供大语言模型在生成代码时所需要的完整依赖关系，而是让模型自行搜索，因此无法区分大语言模型搜索依赖的能力较差还是其代码生成能力本身较差。另一方面，codereval和DevEval提供了完整的依赖关系，但未包括无用和混淆的依赖关系，因此这样提供的依赖关系可能会引导大模型生成代码，从而导致测试结果不公平。此外，之前的基准测试与Humaneval进行比较以证明其有效性。然而，由于这些基准测试要生成的代码长度与Humaneval的代码长度分布并不一致，这种比较本身是不公平的，因此，无法准确反映基准测试的有效性。



Is Your Code Generated by ChatGPT Really Correct? Rigorous Evaluation of Large Language Models for Code Generation
~\cite{liu2023your}

SWE-bench: Can Language Models Resolve Real-World GitHub Issues?
~\cite{jimenez2023swe}

Security Weaknesses of Copilot-Generated Code in GitHub
~\cite{fu2023security}


Classeval: A manually-crafted benchmark for evaluating llms on class-level code generation
~\cite{du2023classeval}
\end{comment}


\subsection{Novelty of Our Study}

Unlike traditional algorithmic problem-based evaluation methods, we used code generation tasks from real projects as evaluation benchmarks, on which we rewrote the functional descriptions and code with obfuscation at different difficulty levels to mitigate the risk of data leakage in existing test benchmarks. In addition, we performed rigorous manual checks on the functionally correct code generated by LLM. Although these code meet the functional requirements, we found some non-functional code quality issues in them, such as deficiencies in maintainability, efficiency, and security, thus revealing the limitations of LLM in terms of code generation quality.

% 与传统基于算法问题的评估方法不同，我们采用了真实项目中的代码生成任务作为评估基准，并在此基础上对功能描述和代码进行了不同难度级别的混淆重写，以缓解现有测试基准中存在的数据泄露风险。此外，我们对LLM生成的功能正确代码进行了严格的人工检查。尽管这些代码符合功能要求，但我们还是在其中发现了一些非功能性代码质量问题，例如可维护性、效率和安全性方面的缺陷，从而揭示了LLM在代码生成质量方面的局限性。






% 首先，与传统基于算法问题的评估方法不同，我们选择了从真实项目中进行代码生成任务的评估。我们从 GitHub 上收集了星级较高的 C 语言项目，并从中选取了被官方测试套件覆盖到的函数作为测试样本。针对每个函数，我们提取了原始文档字符串（即函数的自然语言描述）、函数名称和签名、以及代码实现，形成了一个函数级任务。通过程序依赖性分析，我们确定了每个函数所需的全部上下文依赖，包括必要的 API 调用、结构体和宏等，并添加了一些无用的依赖关系进行混淆，以确保测试结果的公平性，防止模型受到指导。

% 其次，为了降低数据泄露的风险（即我们所收集的函数代码很有可能被大型语言模型用作训练数据），我们邀请了 13 名经验丰富的工程师对功能描述和代码进行了不同难度级别的混淆重写，以减轻模型依赖已见过的正确答案的情况。我们采用了三种代码混淆策略：符号混淆、结构混淆和语义混淆，并将它们结合起来以增加代码的混淆程度。

% 为了自动评估代码生成模型，在\datasetO 中使用了编译通过率和测试通过率来分别评估生成代码的语法正确性和功能正确性。由于\datasetO涉及上下文依赖，因此我们构建了一个项目级执行平台，提供了一个现成的运行时环境，可以自动评估生成代码的功能正确性。我们基于Docker开发了这个平台，为所有项目克隆并建立了环境。给定一个模型生成的多个解决方案，并能够自动将生成的代码放置在适当位置，以模拟实际开发场景。

% 我们在\datasetO上对三种先进的代码生成模型( CodeGen 、StarCoder、ChatGPT )进行了全面的评估，并与HumanEval进行了比较。在评估中，针对每个模型，我们分析了其在代码生成和代码补全场景中的有效性，以及在不同混淆策略下的表现。
% 此外，我们发现，即使通过测试，由大型语言模型生成的代码仍可能存在非功能性代码质量问题，如可维护性和性能。因此，我们对生成的代码进行了手动检查，并对语法问题和非功能性代码质量问题进行了分析，为开发人员提供改进建议。这一研究旨在为开发人员使用大型语言模型生成的代码提供质量检查和改进的方向。





% {\color{red}
% }

==> experiment.tex <==
\section{Results and analysis}
\label{sec:experiments}
In this section, we detail the experiment results and analysis for CodeGen, starCoder, and ChatGPT on CoderEval.

\subsection{\noindent\textbf{RQ1: How do large language models perform in terms of pass rates for the code they generate in the two cases of code that they are exposed to during training versus new code that they are not exposed to?}}



%开源大模型，在模型生成的代码并不是我们所要的代码，即使是通过指令微调的模型，在输入的上下文较多时，模型不能够正确的听从指令。比如wizardCoder，在681条数据中，只有59个是生成了代码的，且这59个里只有22个是我们所要求其生成的目标函数。比如 模型会忽略掉我们已经给出的函数定义，自己根据输入改变函数的名字，我们给出的函数定义为ACLDescribeUser，其生成的函数名为generate_acl_description。



Typically, the training data for LLMs is crawled from the Internet and is closed source. Consequently, there is a risk of data leakage where several projects used to build ConfuEval may be included in the training data. 

% 通常情况下，LLM 的训练数据是从互联网上抓取的，而且是闭源的。因此，训练数据中可能包含用于构建 ConfuEval 的多个项目，存在数据泄露的风险。
% 即使之前的benchmark手工编写了测试用例所有的需求，但模型已经看到过目标生成的代码，模型只需要根据输入的需求匹配到其之前


% 表2中展示了模型在见过的数据上和没见过的数据上的pass1和pass5结果，
% gpt-4-0125和gpt-4-1106-preview比较  gpt-4-0125见过这部分数据


%大型语言模型在代码生成基准测试中表现良好可能仅仅是因为其已经在训练阶段接触过目标代码。


%加一个CoderEval中的表三，对应我们的数据集的模型的结果和在humaneval上的结果。

\vspace{0.6cm}
\begin{tcolorbox}[width=1.0\linewidth, title={}]
\textbf{Summary for RQ1:} 
......
\end{tcolorbox}



% Table generated by Excel2LaTeX from sheet 'RQ1'
\begin{table}[htbp]
  \centering
  \caption{Overall effectiveness of three models on two benchmarks}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{\textbf{Project}}} & \multirow{2}[2]{*}{\textbf{Model}} & \multicolumn{4}{c}{\textbf{in train}} & \multicolumn{4}{c}{\textbf{not in train}} \\
          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{CR1}} & \multicolumn{1}{c}{\textbf{TPR1}} & \multicolumn{1}{c}{\textbf{CR5}} & \multicolumn{1}{c}{\textbf{TPR5}} & \multicolumn{1}{c}{\textbf{CR1}} & \multicolumn{1}{c}{\textbf{TPR1}} & \multicolumn{1}{c}{\textbf{CR5}} & \multicolumn{1}{c}{\textbf{TPR5}} \\
    \midrule
    \multicolumn{1}{c}{\multirow{3}[2]{*}{redis}} & ChatGPT &       & 47.26\% &       & 67.21\% &       & 10.40\% &       & 9.15\% \\
          & CodeGen &       & 15.72\% &       & 19.20\% &       & 2.49\% &       & 1.90\% \\
          & StarCoder &       & 14.85\% &       & 21.85\% &       & 2.12\% &       & 1.54\% \\
    \midrule
    \multicolumn{1}{c}{\multirow{3}[2]{*}{lvgl}} & ChatGPT &       & 39.15\% &       & 42.46\% &       & 11.04\% &       & 8.44\% \\
          & CodeGen &       & 13.24\% &       & 18.15\% &       & 3.90\% &       & 1.95\% \\
          & StarCoder &       & 11.52\% &       & 14.52\% &       & 3.25\% &       & 2.60\% \\
    \midrule
    \multicolumn{1}{c}{\multirow{3}[2]{*}{libvips}} & ChatGPT &       & 43.56\% &       & 49.51\% &       & 8.03\% &       & 6.35\% \\
          & CodeGen &       & 9.45\% &       & 13.42\% &       & 2.34\% &       & 1.67\% \\
          & StarCoder &       & 10.14\% &       & 14.51\% &       & 2.01\% &       & 1.34\% \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:effectiveness}%
\end{table}%



\subsection{\noindent\textbf{RQ2: How does the LLM perform on confused test cases?}}
%为了更好的控制待生成代码的长度，我们采用了代码补全的形式。
%语义混淆补全的时候，如果如果代码不超过20行，就补全一半，如果超过20行就补全后十行


%大语言模型在经过混淆的测试用例上的性能表现如何？

%如果在测试中添加了代码片段，但大模型的代码生成通过率并没有提高，这可能表明大模型更侧重于搜索整合而不是直接根据提示生成代码。大型语言模型在生成代码时通常会通过搜索相关的信息，整合不同的语境和片段来完成任务。即便给予更多信息，模型可能更倾向于从已见过的内容中进行搜索和组合，而不是仅仅根据提示生成全新的代码。 这也强调了模型在生成代码时可能更依赖于其训练集中已有的知识，而非完全根据提示进行创造性的生成。这对于理解大模型的工作方式和生成策略具有重要启示。 
%大模型可能更多地依赖搜索整合的策略，而非根据提示生成代码。这可能意味着模型更倾向于在已有的训练样本中搜索相似片段，而非根据提示独立生成新代码。 
%分析大模型生成的样本，查看生成的代码片段是否与训练集中的片段相似，以确认模型的生成策略。 








%1、selection，从上下文中选择和问题相关的事实，作为回答问题的证据/原因。
%2、Inference，际遇选择出的证据进行推理，看能否回答问题，如果能回答问题，则把推理结果作为新的事实补充道上下文中，回到第一步。

%两倍的上下文和三倍的上下文，模型的能力区别，从而突出精简的上下文的重要性，???




\begin{table*}[htbp]
  \centering
  \caption{Large Models in Code Generation Scenarios Performance}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccccccccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{\textbf{Repo Owner}}} & \multirow{2}[2]{*}{\textbf{Model}} & \multicolumn{4}{c}{\textbf{Symbol Confusion}} & \multicolumn{4}{c}{\textbf{Structural Confusion}} & \multicolumn{4}{c}{\textbf{Symbol Confusion+Structural Confusion}} \\
          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{CR1}} & \multicolumn{1}{c}{\textbf{TPR1}} & \multicolumn{1}{c}{\textbf{CR5}} & \multicolumn{1}{c}{\textbf{TPR5}} & \multicolumn{1}{c}{\textbf{CR1}} & \multicolumn{1}{c}{\textbf{TPR1}} & \multicolumn{1}{c}{\textbf{CR5}} & \multicolumn{1}{c}{\textbf{TPR5}} & \multicolumn{1}{c}{\textbf{CR1}} & \multicolumn{1}{c}{\textbf{TPR1}} & \multicolumn{1}{c}{\textbf{CR5}} & \multicolumn{1}{c}{\textbf{TPR5}} \\
    \midrule
    \multicolumn{1}{c}{\multirow{3}[2]{*}{redis}} & ChatGPT &       & 13.24\% &       & 18.52\% &       & 13.24\% &       & 18.52\% &       & 5.15\% &       & 7.40\% \\
          & CodeGen &       & 1.90\% &       & 2.49\% &       & 1.90\% &       & 2.49\% &       & 0.00\% &       & 0.00\% \\
          & StarCoder &       & 1.54\% &       & 2.12\% &       & 1.54\% &       & 2.12\% &       & 0.00\% &       & 0.00\% \\
    \midrule
    \multicolumn{1}{c}{\multirow{3}[2]{*}{lvgl}} & ChatGPT &       & 8.44\% &       & 11.04\% &       & 8.44\% &       & 11.04\% &       & 4.44\% &       & 6.04\% \\
          & CodeGen &       & 1.95\% &       & 3.90\% &       & 1.95\% &       & 3.90\% &       & 0.00\% &       & 0.00\% \\
          & StarCoder &       & 2.60\% &       & 3.25\% &       & 2.60\% &       & 3.25\% &       & 0.00\% &       & 0.00\% \\
    \midrule
    \multicolumn{1}{c}{\multirow{3}[2]{*}{libvips}} & ChatGPT &       & 6.35\% &       & 8.03\% &       & 6.35\% &       & 8.03\% &       & 3.35\% &       & 4.03\% \\
          & CodeGen &       & 1.67\% &       & 2.34\% &       & 1.67\% &       & 2.34\% &       & 0.00\% &       & 0.00\% \\
          & StarCoder &       & 1.34\% &       & 2.01\% &       & 1.34\% &       & 2.01\% &       & 0.00\% &       & 0.00\% \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:Generation}%
\end{table*}%





% Table generated by Excel2LaTeX from sheet 'RQ2'
\begin{table*}[htbp]
  \centering
  \caption{Large Models in Code Completion Scenarios Performance}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccccccccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{\textbf{Repo Owner}}} & \multirow{2}[2]{*}{\textbf{Model}} & \multicolumn{4}{c}{\textbf{Symbol Confusion}} & \multicolumn{4}{c}{\textbf{Structural Confusion}} & \multicolumn{4}{c}{\textbf{Symbol Confusion+Structural Confusion}} \\
          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{CR1}} & \multicolumn{1}{c}{\textbf{TPR1}} & \multicolumn{1}{c}{\textbf{CR5}} & \multicolumn{1}{c}{\textbf{TPR5}} & \multicolumn{1}{c}{\textbf{CR1}} & \multicolumn{1}{c}{\textbf{TPR1}} & \multicolumn{1}{c}{\textbf{CR5}} & \multicolumn{1}{c}{\textbf{TPR5}} & \multicolumn{1}{c}{\textbf{CR1}} & \multicolumn{1}{c}{\textbf{TPR1}} & \multicolumn{1}{c}{\textbf{CR5}} & \multicolumn{1}{c}{\textbf{TPR5}} \\
    \midrule
    \multicolumn{1}{c}{\multirow{3}[2]{*}{redis}} & ChatGPT &       & 13.24\% &       & 18.52\% &       & 13.24\% &       & 18.52\% &       & 5.15\% &       & 7.40\% \\
          & CodeGen &       & 1.90\% &       & 2.49\% &       & 1.90\% &       & 2.49\% &       & 0.00\% &       & 0.00\% \\
          & StarCoder &       & 1.54\% &       & 2.12\% &       & 1.54\% &       & 2.12\% &       & 0.00\% &       & 0.00\% \\
    \midrule
    \multicolumn{1}{c}{\multirow{3}[2]{*}{lvgl}} & ChatGPT &       & 8.44\% &       & 11.04\% &       & 8.44\% &       & 11.04\% &       & 4.44\% &       & 6.04\% \\
          & CodeGen &       & 1.95\% &       & 3.90\% &       & 1.95\% &       & 3.90\% &       & 0.00\% &       & 0.00\% \\
          & StarCoder &       & 2.60\% &       & 3.25\% &       & 2.60\% &       & 3.25\% &       & 0.00\% &       & 0.00\% \\
    \midrule
    \multicolumn{1}{c}{\multirow{3}[2]{*}{libvips}} & ChatGPT &       & 6.35\% &       & 8.03\% &       & 6.35\% &       & 8.03\% &       & 3.35\% &       & 4.03\% \\
          & CodeGen &       & 1.67\% &       & 2.34\% &       & 1.67\% &       & 2.34\% &       & 0.00\% &       & 0.00\% \\
          & StarCoder &       & 1.34\% &       & 2.01\% &       & 1.34\% &       & 2.01\% &       & 0.00\% &       & 0.00\% \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:Generation}%
\end{table*}%




\vspace{0.6cm}
\begin{tcolorbox}[width=1.0\linewidth, title={}]
\textbf{Summary for RQ2:} 
......
\end{tcolorbox}



\subsection{\noindent\textbf{RQ3: What are the common issues in ChatGPT-generated code?}}



%不同模型的错误分布
%举例wizardCoder生成的目标函数不是我们要的目标函数。
%有多少不能够正常生成代码，有多少生成的代码和目标函数不一致，有多少生成的代码编译错误，测试错误。


\subsubsection{Syntax Errors}

We further analyzed the code that failed to compile. To this end, we automatically parsed the error logs generated during interpretation and execution and presented the distribution of all syntax errors in Table ~\ref{tab:errorCategories}.
From these syntax errors and their proportions, it is clear that the big model performs relatively poorly in handling function and type declaration errors, especially the high proportion of errors in implicitly declared functions and type conflicts, which amounted to 26.57\% and 11.61\%. This may indicate that the large model has some difficulties in understanding and handling function and type declarations, resulting in a high error rate when generating code.

In addition, the large model also performs poorly in terms of data structure and member access errors, especially the error handling of non-existing structure members, with a high error rate of 17.28\%. This may imply that the large model has some challenges in understanding and manipulating data structures, which may lead to frequent data structure access errors during code generation.

Furthermore, for syntax errors involving assignment and pointer operations, such as converting integers to pointers without forced conversion, incompatible pointer types, and incorrect use of arrays or pointers, the Big Model also had a certain percentage of errors, which may reflect its shortcomings in handling type conversion and pointer operations.

In summary, the big model is relatively weak in handling function and type declarations, data structure access, and pointer manipulation. To address these weaknesses, the training and optimization of the Big Model in the field of software engineering can be further strengthened to improve its understanding of code structure and syntax, thus improving the quality and accuracy of the generated code.


% 我们进一步分析了未能通过编译的代码。为此，我们自动解析解释和执行过程中产生的错误日志，并在表5中呈现所有语法错误的分布。
% 具体来说，我们发现大多数错误地代码都


~\figurename~\ref{fig:syntaxIssues} shows examples of syntax errors in the code generated by ChatGPT. First, we notice that the number of parameters passed in the call to the expandIfNeeded function is insufficient. Although the expandIfNeeded function is declared to accept three arguments, only two arguments are provided in the actual call. This suggests that the model may have some difficulty in understanding the context of the function call, and may not be able to correctly recognize the signature of the function and how it is called. Secondly, the generated code tries to access a non-existent member 'lastAccessTime' of the structure 'robj'. This suggests that the model has some deficiencies in understanding how structures are organized and how members are accessed, and may not be able to accurately capture the definition and usage of structure members.

% 结构体成员的访问准确性
% 参数数量和类型匹配的能力不足


% 从这些语法错误及其比例来看，大模型在处理函数和类型声明错误方面的表现相对较差，尤其是隐式声明函数和类型冲突的错误比例较高，达到了26.57%和11.61%。这可能表明大模型在理解和处理函数和类型声明方面存在一定的困难，导致在生成代码时出现了较高的错误率。

% 另外，在数据结构和成员访问错误方面，大模型也表现不佳，特别是对不存在的结构成员的错误处理，错误比例高达17.28%。这可能暗示了大模型在理解和操作数据结构方面存在一定的挑战，可能导致在代码生成过程中频繁出现数据结构访问错误。

% 此外，对于语法错误中涉及到赋值和指针操作的错误，如将整数转换为指针而没有进行强制转换、不兼容的指针类型、以及不正确的使用数组或指针等，大模型也存在一定的错误比例，这可能反映了其在处理类型转换和指针操作时的不足之处。

% 综上所述，大模型在处理函数和类型声明、数据结构访问以及指针操作等方面的能力相对较弱。针对这些薄弱点，可以进一步加强大模型在软件工程领域的训练和优化，提高其对代码结构和语法的理解能力，从而改善生成代码的质量和准确性。
%图5展示了ChatGPT生成的代码中存在的语法错误示例。首先，我们注意到在调用expireIfNeeded函数时，传递的参数数量不足。虽然expireIfNeeded函数被声明为接受三个参数，但在实际调用时只提供了两个参数。这表明模型在理解函数调用上下文时可能存在一定困难，可能无法正确识别函数的签名和调用方式。其次，生成的代码尝试访问结构体robj的一个不存在的成员lastAccessTime。这表明模型在理解结构体的组织和成员访问方式方面存在一定缺陷，可能无法准确捕获结构体成员的定义和用法。




\begin{figure}[htbp]
	\centering
    \vspace{-1mm}
	\includegraphics[width=0.4\textwidth]{figs/syntaxError.pdf}
	\caption{Examples of syntax issues with model-generated code. There are two syntax errors in this code, a function passing too few parameters and a call to a non-existent struct member.}
    \vspace{-1mm}
	\label{fig:syntaxIssues}
\end{figure}   




\subsubsection{Non-functional code quality issues}

We further analyzed the code generated by the large-scale language model and found that even though the code passed integration tests, there were still some non-functional code quality issues.
These issues may include, but are not limited to, poor readability of the code, poor performance, security vulnerabilities,  and so on. Although these issues may not directly affect the proper functioning of the code, they potentially suggest several potential threats and risks. For example, poor performance may lead to delayed system response time, affecting user experience and overall performance. Security vulnerabilities may be exploited by malicious attackers, resulting in data leakage or system paralysis.

To gain a comprehensive understanding of the non-functional code quality issues present in the code generated by ChatGPT, we conducted a manual analysis and categorized these issues to better identify areas of improvement for ChatGPT. While performing the analysis, we found that a single generated code snippet could have multiple issues simultaneously, which interacted with each other and added to the complexity of the analysis. By pinpointing and highlighting these issues, our analysis can not only provide important guidance for future research and development of code generators but also provide developers with directions for checking the quality and reliability of generated code when working with code generated from large-scale models.

Table~\ref{tab:qualityIssues} lists the non-functional code quality issues that we found in our code, mainly in the areas of configuration parsing, resource management, code logic, and error handling. These problems include improper configuration parsing, memory and file mismanagement in resource management, insufficient boundary condition handling inefficient code in code logic, and insufficient error detection, incomplete error handling, and inadequate error feedback in error handling.


~\figurename~\ref{fig:testCase} illustrates an example of an underperformance problem. In the correct code, a conditional statement is used to determine whether the character c is in the range '0' to '9', 'a' to 'f', or 'A' to 'F', and the corresponding hexadecimal number is computed based on the value of the character. This implementation is much more concise and readable. In the generated code, the switch statement determines the value of character c one by one and returns the corresponding hexadecimal number. This implementation can be executed correctly, but it is lengthy and complex compared to the correct code, making it less readable and maintainable. 
In this example in the top right of~\figurename~\ref{fig:testCase}, the code generated by the Big Model lacks a check to see if the pointer 'myself' is null, which could lead to a program crash or undefined behavior triggered by accessing the pointer when it has not been initialized or released.
In this example in the bottom right of~\figurename~\ref{fig:testCase}, the code generated by the big model directly returns the error code C\_ERR when a file open fails, without any detailed handling or logging of the error. In practice, if a file open fails, there may be a variety of reasons, such as the file does not exist, insufficient permissions, etc. A direct return of the error code is not sufficient to indicate the specific cause of the problem, and it does not provide the developer with enough information to troubleshoot and repair the problem.



%改为classeval中的扇形图

\begin{table*}[htbp]
  \centering
  \caption{Code Syntax Problems}
  \vspace{-1mm}
  \begin{center}
       \setlength{\tabcolsep}{1mm}{
        \resizebox{1\textwidth}{!}{
    \begin{tabular}{ccc}
    \toprule
        \multicolumn{1}{c}{\textbf{Category}} & \multicolumn{1}{c}{\textbf{Sub-category}} & \multicolumn{1}{c}{\textbf{Proportion}} \\

    \midrule
    \multirow{4}[2]{*}{Function and Type Declaration Errors} & Implicit declaration of function & 26.57\% \\
          & Undeclared type & 0.27\% \\
          & Type conflict & 11.61\% \\
          & API parameter count mismatch & 0.89\% \\
    \midrule
    \multirow{4}[2]{*}{Type Conversion and Assignment Errors} & Making a pointer from an integer without a cast & 7.45\% \\
          & Incompatible pointer type & 1.09\% \\
          & Incompatible type assignment & 1.30\% \\
          & Redefinition & 1.30\% \\
    \midrule
    \multirow{2}[2]{*}{Scope and Definition Errors} & Conflict between static and non-static declarations & 1.30\% \\
          & ncorrect access to structure or union member & 0.34\% \\
    \midrule
    \multirow{3}[2]{*}{Data Structure and Member Access Errors} & Nonexistent structure member & 17.28\% \\
          & Misuse of structure pointer & 5.74\% \\
          & Attempt to access a member of an integer type with the '->' operator & 0.20\% \\
    \midrule
    \multirow{8}[2]{*}{Syntax Errors} & Missing necessary expression inside parentheses, or extraneous closing parenthesis & 0.55\% \\
          & Invalid binary operands & 0.48\% \\
          & Incorrect use of array, pointer, or vector & 1.50\% \\
          & Array subscript is not an integer & 0.20\% \\
          & Subscripted value is pointer to function & 0.20\% \\
          & Assignment to expression with array type & 0.55\% \\
          & Lvalue required as the left operand of assignment & 5.74\% \\
          & Expected expression error & 0.41\% \\
    \bottomrule
    \end{tabular}%
        }} 
 \end{center}
  \label{tab:errorCategories}%
\end{table*}%




\begin{table}[htbp]
  \centering
  \caption{Non-functional code quality issues}
  \vspace{-1mm}
  \begin{center}
       \setlength{\tabcolsep}{1mm}{
        \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{ccc}
    \toprule
    \textbf{Category} & \multicolumn{1}{p{11.625em}}{\textbf{Sub-category}} & \textbf{Proportion} \\
    \midrule
    Configuration Analysis & Improper configuration parsing & XX\% \\
    \midrule
    \multirow{2}[2]{*}{Resource Management} & Improper memory management & XX\% \\
          & Improper file management & XX\% \\
    \midrule
    \multirow{2}[2]{*}{Code Logic} & Poor boundary condition handling & XX\% \\
          & Inefficient code & XX\% \\
    \midrule
    \multirow{3}[2]{*}{Error Handling} & Inadequate error detection & XX\% \\
          & Incomplete error handling & XX\% \\
          & Inadequate error feedback & XX\% \\
    \bottomrule
    \end{tabular}%
        }} 
 \end{center}
  \label{tab:qualityIssues}%
\end{table}%








\begin{figure*}[htbp]
	\centering
    \vspace{-1mm}
	\includegraphics[width=0.9\textwidth]{figs/testCase.pdf}
	\caption{Examples of non-functional code quality issues with model-generated code}
    \vspace{-1mm}
	\label{fig:testCase}
\end{figure*}   


%
\begin{comment}
对于上下文相关错误的定义，除了私有库的API调用错误和结构体成员变量使用错误之外，还需要考虑其他可能的错误类型。例如，对于项目中的依赖关系管理、错误处理逻辑、特定业务规则的遵循等方面的错误。“库相关错误”、“项目配置错误”、“业务逻辑错误”等
私有库API调用错误可能由于多种原因，如API的不当使用、参数不匹配或者对库的更新不知情等。同样，结构体成员变量使用错误可能涉及对数据结构不当修改、访问控制违规或者类型不兼容等问题。

API调用错误：

错误使用API函数，包括错误的参数或参数顺序。
对废弃的API的调用或未遵守新的API设计模式。
API使用时对版本兼容性的忽略。

库和框架集成问题：
错误地集成或更新第三方库和框架。
对库内数据结构和算法的错误假设。
忽略特定库的初始化和配置步骤。

结构体和数据类型使用错误：
结构体成员的错误访问（例如访问私有成员）。
类型定义（typedef）的不一致使用。
指针和数组的不当操作，可能导致内存泄漏或越界。

多线程和并发问题：
死锁、竞态条件和其他同步问题。
对全局变量的不安全访问。
线程间通信的逻辑错误。
内存管理错误：

动态分配内存未正确释放，造成内存泄漏。
使用未初始化或已释放的内存。
错误的内存分配大小或对齐问题。

环境依赖问题：
代码依赖于特定的操作系统或硬件特性。
编译器特定的行为或预处理器指令的错误使用。
对环境变量的错误假设或使用。

构建和配置问题：
Makefile或其他构建脚本中的错误。
对编译器标志或链接选项的错误配置。
忽略跨平台构建的要求。

安全漏洞：
缓冲区溢出或格式字符串漏洞。
不安全的数据传输或错误的加密实现。
授权和认证机制的不当实施。

业务逻辑错误：
与项目需求不符的逻辑实现。
对业务规则的误解或错误实现。
忽略项目特定的约定或流程。

代码风格和规范：
未遵守项目的代码风格和命名约定。
文档注释不全或不准确，影响代码可读性和维护性。

版本控制和协作问题：
代码合并中的冲突没有正确解决。
分支管理的策略错误或不一致。

\end{comment}



%ChatGPT Prompt Patterns for Improving Code Quality, Refactoring, Requirements Elicitation, and Software Design
%可以模仿这篇论文的论证思路提出我们的模板，然后来验证

\vspace{0.6cm}
\begin{tcolorbox}[width=1.0\linewidth, title={}]
\textbf{Summary for RQ3:} 
 Wrong Outputs Code Style & Maintainability issues are the most common challenges faced by the ChatGPT-generated code while Compilation & Runtime Errors and Performance & Efficiency issues are relatively less prevalent.
\end{tcolorbox}




